TextureSAM: Towards a Texture Aware Foundation Model for Segmentation

Segment Anything Models (SAM) have achieved remarkable success in object segmentation tasks across diverse datasets. However, these models are predominantly trained on large-scale semantic segmentation datasets, which introduce a bias toward object shape rather than texture cues in the image. This limitation is critical in domains such as medical imaging, material classification, and remote sensing, where texture changes define object boundaries. In this study, we investigate SAM's bias toward semantics over textures and introduce a new texture-aware foundation model, TextureSAM, which performs superior segmentation in texture-dominant scenarios. To achieve this, we employ a novel fine-tuning approach that incorporates texture augmentation techniques, incrementally modifying training images to emphasize texture features. By leveraging a novel texture-alternation of the ADE20K dataset, we guide TextureSAM to prioritize texture-defined regions, thereby mitigating the inherent shape bias present in the original SAM model. Our extensive experiments demonstrate that TextureSAM significantly outperforms SAM-2 on both natural (+0.2 mIoU) and synthetic (+0.18 mIoU) texture-based segmentation datasets. The code and texture-augmented dataset will be publicly available.

==> CNT.tex <==
To texturize an image, we embed both the texture and the image into latent space, interpolate and decode it back.
Formally, the autoencoder architecture, with encoder $\encoder$ and the decoder $\decoder$, represents a texture $\image$ as a composition of 2D Gaussians $\gaussianset=\setof{\gaussian}=\encoder(\image)$.
$\encoder$ takes images of size $\imagesize\times\imagesize$ and $\decoder$ is fully convolutional. $\imagesize=128$.
A Gaussian $\gaussian=\setof{\gaussiancenter,\gaussiancovariance,\appearancefeature}$ including its center $\gaussiancenter$ and covariance $\gaussiancovariance$ along with an appearance feature $\appearancefeature$, represents a texton that is the basic element in texture perception ~\cite{Julesz:1981:TET}.
As $\gaussiancenter$ and $\gaussiancovariance$ encode the position and shape of a texton, $\appearancefeature$ encodes appearance of it. Altering the feature $\appearancefeature$ results in altered appearance of the texton.
For more details about the texture model, please refer to the original paper ~\cite{Tu:2024:CNT}.

% \shai{peihan, please lead with an overview. "We use an auto-encoder to represent texture as a Gaussian Mixture Model. To texturize an image, we embed both the texture and the image into latent space, interpolate and decode it back" and then continue to describe the method in more details.}
% \peihan{(Feb 21, 2024)
% Thanks for the feedback. I have modified the writings. Please let me know if it needs to be further improved. (Feel free to comment out my comments/replies that have been addressed.)
% }%peihan

To texturize an image $\contentimage$, for each instance mask $\mask$, we randomly select a texture $\textureimage$ from a unused category in DT dataset (if all categories are used, randomly select a texture from the entire dataset).
Before further processing, we scale the content image $\contentimage$ into $8\imagesize\times8\imagesize$ pixels and the texture image $\textureimage$ into $\imagesize\times\imagesize$ pixels.
Since the model focuses solely on texture, we extract overlapping patches $\contentimagepatch$ of size $\imagesize\times\imagesize$ with spacing of $3/4\imagesize$ pixels from $\contentimage$, $\patch \in \patchset=\setof{0,1,2,...,\numpatches}$ -- treating every patch as an independent texture sample.
$\contentimagepatch$ is then encoded into a composition of Gaussians $\gaussiansetcontentpatch$, and these representations are merged in their original spatial order to produce Gaussians $\gaussiansetcontent=\merge(\bigcup_{\patch \in \patchset}\gaussiansetcontentpatch)$ reconstructed as the original image. $\merge$ merges overlapping patches of Gaussians while ensuring smooth transition (see \cite{Tu:2024:CNT} for details).
Each texture $\textureimage$ is also encoded as Gaussians $\gaussiansettexture=\setof{\gaussiantexture}$ by directly forwarding them through the encoder $\encoder$.
To alter texture within a binary instance mask $\mask \in \maskset$, we select Gaussians centered within the mask $\contentmasked{\gaussianset}=\setof{\contentmasked{\gaussian}}=\setof{\gaussiancontent | \gaussiancontent \in \gaussiansetcontent, \mask(\gaussiancenter_\contentsymbol)=1}$ and modulate their appearance features $\contentmasked{\appearancefeature} \in \contentmasked{\gaussian}$. For each $\contentmasked{\appearancefeature}$, we randomly pick a feature $\appearancefeature_\texturesymbol \in \gaussiantexture$ from $\gaussiansettexture$, the modified feature $\contentmasked{\modified{\appearancefeature}}$ is computed as
\begin{align}
\contentmasked{\modified{\appearancefeature}}&=\interpcoefficient \contentmasked{\appearancefeature} + (1-\interpcoefficient) \appearancefeature_\texturesymbol.
\end{align}

$\interpcoefficient \in [0, 1]$ is the interpolation coefficient.
The modified Gaussian is
$\contentmasked{\modified{\gaussian}}=  \setof{\contentmasked{\modified{\appearancefeature}},\contentmasked{\gaussiancenter},\contentmasked{\gaussiancovariance}}$, where $\contentmasked{\gaussiancenter}\in \gaussiantexture$, $\contentmasked{\gaussiancovariance} \in \gaussiantexture$.
The modified Gaussians of the content image are the union of modified Gaussians within masks $\contentmasked{\modified{\gaussianset}}$
\begin{align}
\modified{\gaussianset_\contentsymbol}= \bigcup_{\mask \in \maskset} \contentmasked{\modified{\gaussianset}},
\end{align}
the textured content image is decoded as  $\modified{\contentimage}=\decoder(\modified{\gaussianset_\contentsymbol})$.
Finally, $\modified{\contentimage}$ is scaled back to its original size.

We vary $\interpcoefficient$ from 0.0 to 1.0 in increments of 0.1, giving 11 equally spaced values: 0.0, 0.1, ..., 1.0. For each content image $\contentimage$, we generate 11 texturized images. The textured-ADE20K dataset include $25574 \times 11=303314$ images in total.
% Algorithm \ref{alg:dataset} summarize the dataset creation process in pseudocode.
% Fig. \ref{fig:texture_transfer_method} illustrates the process of generating one augmented, textured dataset image.

% Please refer the supplemental material for a visualization of generating one augmented, textured dataset image.

% \paragraph{Discussion}
% When $\interpcoefficient=0$, $\modified{\contentimage}$ is the \emph{texturization} of $\contentimage$: $\modified{\contentimage}$ closely matches $\contentimage$ but is not the exact reconstruction (Fig.~\ref{fig:dataset_samples}, rows: 1-2, columns: 1-2).
% This is because we encode $\contentimage$ as Gaussians using $\encoder$ patch-by-patch and reconstruct them using $\decoder$, which 1) projects each image patch onto the learned texture space 2) merges overlapping Gaussian patches and 3) reconstruct Gaussians as $\modified{\contentimage}$.
% Intuitively, this process 1) finds closest texture embeddings for image patches 2) spatially merge texture embeddings to ensure smooth transition and 3) reconstruct images from blended textures.


% \peihan{(Feb 9, 2025) Let me know if we need to improve the discussions here based on assumptions made in experiments.}



% \input{pseudocode_dataset}
% \input{figs/texture_transfer_method}


==> figs/dataset_sample_OLD.tex <==
\begin{figure*}[htbp]
    \centering
    \captionsetup[subfloat]{labelformat=empty}
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree0.0_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree0.2_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree0.4_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree0.6_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree0.8_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/transportation/cargo_deck__airplane/ADE_train_00005115_seg.png}
    }%
    
    \vspace{-0.8cm}

    \subfloat[Original]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597.jpg}
    }%
    \subfloat[$\interpcoefficient=0.0$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree0.0_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=0.2$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree0.2_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=0.4$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree0.4_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=0.6$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree0.6_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=0.8$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree0.8_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=1.0$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[Instance masks]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/urban/city/ADE_train_00005597_seg.png}
    }%
    
    \vspace{-0.3cm}
    
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/nature_landscape/cliff/ADE_frame_00000109.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/nature_landscape/cliff/ADE_frame_00000109_textured/textured_degree0.5_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/nature_landscape/cliff/ADE_frame_00000109_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/nature_landscape/cliff/ADE_frame_00000109_seg.png}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/workspace/cleanroom/ADE_train_00005649.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/workspace/cleanroom/ADE_train_00005649_textured/textured_degree0.5_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/workspace/cleanroom/ADE_train_00005649_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/workspace/cleanroom/ADE_train_00005649_seg.png}
    }%
    
    \vspace{-0.8cm}

    \subfloat[Original]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/home_or_hotel/hotel_room/ADE_train_00009539.jpg}
    }%
    \subfloat[$\interpcoefficient=0.5$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/home_or_hotel/hotel_room/ADE_train_00009539_textured/textured_degree0.5_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=1.0$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/home_or_hotel/hotel_room/ADE_train_00009539_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[Instance masks]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/home_or_hotel/hotel_room/ADE_train_00009539_seg.png}
    }%
    \subfloat[Original]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/cultural/classroom/ADE_frame_00000106.jpg}
    }%
   \subfloat[$\interpcoefficient=0.5$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/cultural/classroom/ADE_frame_00000106_textured/textured_degree0.5_v2.jpg}
    }%
    \subfloat[$\interpcoefficient=1.0$]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/cultural/classroom/ADE_frame_00000106_textured/textured_degree1.0_v2.jpg}
    }%
    \subfloat[Instance masks]{%
    \includegraphics[width=0.12\linewidth]{figs/dataset/training/cultural/classroom/ADE_frame_00000106_seg.png}
    }%

    
    \vspace{-0.2cm}


    \caption{Samples of Textured-ADE20K dataset. Incremental changes in $\eta$ produce gradual change in texture shift for the resulting image. For low $\eta$ values most of the semantic information in the image is retained. For $\eta=1$ the instances are completely shifted towards the target textures.}
    \label{fig:dataset_samples}
\end{figure*}


==> figs/teaser_OLD.tex <==











\begin{figure*}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c c c c c c c c c}
        {\raisebox{3\height}{\textbf{Image}}} &  
        \includegraphics[width=0.1\linewidth]{images/2.jpg} &
        \includegraphics[width=0.1\linewidth]{images/304.jpg} &
        \includegraphics[width=0.1\linewidth]{images/5.jpg} &
        \includegraphics[width=0.1\linewidth]{images/200.jpg} &
        \includegraphics[width=0.1\linewidth]{images/70.jpg} &
        \includegraphics[width=0.1\linewidth]{images/325.jpg} &        
        \includegraphics[width=0.1\linewidth]{images_part2/476.jpg} &            
        \includegraphics[width=0.1\linewidth]{images/78.jpg} \\

        {\raisebox{3\height}{\textbf{SAM}}} &  
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_2.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_304.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_5.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_200.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_70.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_325.jpg} &             
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s_part2/masked_476.jpg} & 
        \includegraphics[width=0.1\linewidth]{natural_images_seg_s/masked_78.jpg} \\

        {\raisebox{3\height}{\textbf{TextureSAM}}} &  
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_2.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_304.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_5.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_200.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_70.jpg} &
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_325.jpg} &   
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3_part_2/masked_476.jpg} &  
        \includegraphics[width=0.1\linewidth]{natural_images_seg_0.3/masked_78.jpg} \\

        {\raisebox{3\height}{\textbf{GT}}} &  
        \includegraphics[width=0.1\linewidth]{labeled_images/2.png} &
        \includegraphics[width=0.1\linewidth]{labeled_images_part2/304.png} &
        \includegraphics[width=0.1\linewidth]{labeled_images/5.png} &
        \includegraphics[width=0.1\linewidth]{labeled_images_part2/200.png} &
        \includegraphics[width=0.1\linewidth]{labeled_images/70.png} &
        \includegraphics[width=0.1\linewidth]{labeled_images_part2/325.png} &  
        \includegraphics[width=0.1\linewidth]{labeled_images_part2/476.png} &            
        \includegraphics[width=0.1\linewidth]{labeled_images/78.png} \\        
    \end{tabular}
    \caption{Examples for segmentation of natural images from the Kaust256 dataset. Compared with the original SAM (2nd row), TextureSAM (3rd row) is more adept at recognizing areas defined by texture changes. SAM's reliance on semantic shape results in fragmented segmentation while TextureSAM provides segmentation of whole areas defined by texture changes. Notice the groundtruth (4th row) annotations mark only one texture change, while TextureSAM predictions include multiple  different textured areas, as can be observed on the  1st and 3rd examples from the left.}
    \label{fig:teaser}
\end{figure*}

==> iccv_OLD.tex <==
% ---------------------------------------------------------------
%
% $Id: iccv.sty,v 1.3 2005/10/24 19:56:15 awf Exp $
%
% by Paolo.Ienne@di.epfl.ch
% some mods by awf@acm.org
%
% ---------------------------------------------------------------
%
% no guarantee is given that the format corresponds perfectly to
% IEEE 8.5" x 11" Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------
% with LaTeX2e:
% =============
%
% use as
%   \documentclass[times,10pt,twocolumn]{article}
%   \usepackage{latex8}
%   \usepackage{times}
%
% ---------------------------------------------------------------

% with LaTeX 2.09:
% ================
%
% use as
%   \documentstyle[times,art10,twocolumn,latex8]{article}
%
% ---------------------------------------------------------------
% with both versions:
% ===================
%
% specify \iccvfinalcopy to emit the final camera-ready copy
%
% specify references as
%   \bibliographystyle{ieee}
%   \bibliography{...your files...}
%
% ---------------------------------------------------------------

\usepackage{eso-pic}
\usepackage{xspace}

\typeout{ICCV 8.5 x 11-Inch Proceedings Style `iccv.sty'.}

% ten point helvetica bold required for captions
% eleven point times bold required for second-order headings
% in some sites the name of the fonts may differ,
% change the name here:
\font\iccvtenhv  = phvb at 8pt % *** IF THIS FAILS, SEE iccv.sty ***
\font\elvbf  = ptmb scaled 1100

% If the above lines give an error message, try to comment them and
% uncomment these:
%\font\iccvtenhv  = phvb7t at 8pt
%\font\elvbf  = ptmb7t scaled 1100

% set dimensions of columns, gap between columns, and paragraph indent
\setlength{\textheight}{8.875in}
\setlength{\textwidth}{6.875in}
\setlength{\columnsep}{0.3125in}
\setlength{\topmargin}{0in}
\setlength{\headheight}{0in}
\setlength{\headsep}{0in}
\setlength{\parindent}{1pc}
\setlength{\oddsidemargin}{-.304in}
\setlength{\evensidemargin}{-.304in}

\newif\ificcvfinal
\iccvfinalfalse
\def\iccvfinalcopy{\global\iccvfinaltrue}

% memento from size10.clo
% \normalsize{\@setfontsize\normalsize\@xpt\@xiipt}
% \small{\@setfontsize\small\@ixpt{11}}
% \footnotesize{\@setfontsize\footnotesize\@viiipt{9.5}}
% \scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
% \tiny{\@setfontsize\tiny\@vpt\@vipt}
% \large{\@setfontsize\large\@xiipt{14}}
% \Large{\@setfontsize\Large\@xivpt{18}}
% \LARGE{\@setfontsize\LARGE\@xviipt{22}}
% \huge{\@setfontsize\huge\@xxpt{25}}
% \Huge{\@setfontsize\Huge\@xxvpt{30}}

\def\@maketitle
   {
   \newpage
   \null
   \vskip .375in
   \begin{center}
      {\Large \bf \@title \par}
      % additional two empty lines at the end of the title
      \vspace*{24pt}
      {
      \large
      \lineskip .5em
      \begin{tabular}[t]{c}
         \ificcvfinal\@author\else Anonymous ICCV submission\\
         \vspace*{1pt}\\%This space will need to be here in the final copy, so don't squeeze it out for the review copy.
Paper ID \iccvPaperID \fi
      \end{tabular}
      \par
      }
      % additional small space at the end of the author name
      \vskip .5em
      % additional empty line at the end of the title block
      \vspace*{12pt}
   \end{center}
   }

\def\abstract
   {%
   \centerline{\large\bf Abstract}%
   \vspace*{12pt}%
   \it%
   }

\def\endabstract
   {
   % additional empty line at the end of the abstract
   \vspace*{12pt}
   }

\def\affiliation#1{\gdef\@affiliation{#1}} \gdef\@affiliation{}

\newlength{\@ctmp}
\newlength{\@figindent}
\setlength{\@figindent}{1pc}

\long\def\@makecaption#1#2{
   \setbox\@tempboxa\hbox{\small \noindent #1.~#2}
   \setlength{\@ctmp}{\hsize}
   \addtolength{\@ctmp}{-\@figindent}\addtolength{\@ctmp}{-\@figindent}
   % IF longer than one indented paragraph line
   \ifdim \wd\@tempboxa >\@ctmp
      % THEN DON'T set as an indented paragraph
      {\small #1.~#2\par}
   \else
      % ELSE center
      \hbox to\hsize{\hfil\box\@tempboxa\hfil}
  \fi}

% correct heading spacing and type
\def\iccvsection{\@startsection {section}{1}{\z@}
   {10pt plus 2pt minus 2pt}{7pt} {\large\bf}}
\def\iccvssect#1{\iccvsection*{#1}}
\def\iccvsect#1{\iccvsection{\hskip -1em.~#1}}
\def\section{\@ifstar\iccvssect\iccvsect}

\def\iccvsubsection{\@startsection {subsection}{2}{\z@}
   {8pt plus 2pt minus 2pt}{6pt} {\elvbf}}
\def\iccvssubsect#1{\iccvsubsection*{#1}}
\def\iccvsubsect#1{\iccvsubsection{\hskip -1em.~#1}}
\def\subsection{\@ifstar\iccvssubsect\iccvsubsect}

%% --------- Page background marks: Ruler and confidentiality

% ----- define vruler
\makeatletter
\newbox\iccvrulerbox
\newcount\iccvrulercount
\newdimen\iccvruleroffset
\newdimen\cv@lineheight
\newdimen\cv@boxheight
\newbox\cv@tmpbox
\newcount\cv@refno
\newcount\cv@tot
% NUMBER with left flushed zeros  \fillzeros[<WIDTH>]<NUMBER>
\newcount\cv@tmpc@ \newcount\cv@tmpc
\def\fillzeros[#1]#2{\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi
\cv@tmpc=1 %
\loop\ifnum\cv@tmpc@<10 \else \divide\cv@tmpc@ by 10 \advance\cv@tmpc by 1 \fi
   \ifnum\cv@tmpc@=10\relax\cv@tmpc@=11\relax\fi \ifnum\cv@tmpc@>10 \repeat
\ifnum#2<0\advance\cv@tmpc1\relax-\fi
\loop\ifnum\cv@tmpc<#1\relax0\advance\cv@tmpc1\relax\fi \ifnum\cv@tmpc<#1 \repeat
\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi \relax\the\cv@tmpc@}%
% \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
\def\makevruler[#1][#2][#3][#4][#5]{\begingroup\offinterlineskip
\textheight=#5\vbadness=10000\vfuzz=120ex\overfullrule=0pt%
\global\setbox\iccvrulerbox=\vbox to \textheight{%
{\parskip=0pt\hfuzz=150em\cv@boxheight=\textheight
\cv@lineheight=#1\global\iccvrulercount=#2%
\cv@tot\cv@boxheight\divide\cv@tot\cv@lineheight\advance\cv@tot2%
\cv@refno1\vskip-\cv@lineheight\vskip1ex%
\loop\setbox\cv@tmpbox=\hbox to0cm{{\iccvtenhv\hfil\fillzeros[#4]\iccvrulercount}}%
\ht\cv@tmpbox\cv@lineheight\dp\cv@tmpbox0pt\box\cv@tmpbox\break
\advance\cv@refno1\global\advance\iccvrulercount#3\relax
\ifnum\cv@refno<\cv@tot\repeat}}\endgroup}%
\makeatother
% ----- end of vruler

% \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
\def\iccvruler#1{\makevruler[12pt][#1][1][3][0.993\textheight]\usebox{\iccvrulerbox}}
\AddToShipoutPicture{%
\ificcvfinal\else
  %\AtTextLowerLeft{%
  % \color[gray]{.15}\framebox(\LenToUnit{\textwidth},\LenToUnit{\textheight}){}
  %}
\iccvruleroffset=\textheight
\advance\iccvruleroffset by -3.7pt
  \color[rgb]{.5,.5,1}
  \AtTextUpperLeft{%
    \put(\LenToUnit{-35pt},\LenToUnit{-\iccvruleroffset}){%left ruler
      \iccvruler{\iccvrulercount}}
    \put(\LenToUnit{\textwidth\kern 30pt},\LenToUnit{-\iccvruleroffset}){%right ruler
      \iccvruler{\iccvrulercount}}
  }
\def\pid{\parbox{1in}{\begin{center}\bf\sf{\small ICCV}\\\#\iccvPaperID\end{center}}}
  \AtTextUpperLeft{%paperID in corners
    \put(\LenToUnit{-65pt},\LenToUnit{45pt}){\pid}
    \put(\LenToUnit{\textwidth\kern-8pt},\LenToUnit{45pt}){\pid}
  }
  \AtTextUpperLeft{%confidential
    \put(0,\LenToUnit{1cm}){\parbox{\textwidth}{\centering\iccvtenhv
       ICCV 2017 Submission \#\iccvPaperID. CONFIDENTIAL REVIEW COPY.  DO NOT DISTRIBUTE.}}
  }
\fi
}

%%% Make figure placement a little more predictable.
% We trust the user to move figures if this results
% in ugliness.
% Minimize bad page breaks at figures
\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.99}
\renewcommand{\topfraction}{0.99}
\renewcommand{\bottomfraction}{0.99}
\renewcommand{\dblfloatpagefraction}{0.99}
\renewcommand{\dbltopfraction}{0.99}
\setcounter{totalnumber}{99}
\setcounter{topnumber}{99}
\setcounter{bottomnumber}{99}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% ---------------------------------------------------------------


==> macro.tex <==
\newcommand{\peihan}[1]{\textcolor{blue}{peihan: #1}}

\newcommand{\shai}[1]
{\textcolor{red}{shai: #1}}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\newcommand\shai[1]{\textcolor{red}{\textbf{SHAI:} #1 }}
\definecolor{green}{rgb}{0.0, 0.5, 0.0}
\newcommand\leo[1]{\textcolor{green}{\textbf{LEO:} #1 }}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


\newcommand{\radiance}{\mathbf{c}}
\newcommand{\nerfparams}{\boldsymbol{\phi}}
\newcommand{\rfield}{\mathcal{R}}
\newcommand{\density}{\tau}
\newcommand{\x}{\mathbf{x}}
\newcommand{\dir}{\mathbf{d}}
\newcommand{\ray}{\mathbf{r}}
\newcommand{\raycolor}{\mathbf{C}}
\newcommand{\image}{\mathbf{I}}
\newcommand{\datasetsize}{\mathbf{N}}
\newcommand{\images}{\mathcal{I}}
\newcommand{\gtcolor}{\mathbf{y}}
\newcommand{\gt}{\text{gt}}
\newcommand{\nRays}{R}


\usepackage{booktabs}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{longtable}

==> pseudocode_dataset.tex <==
\begin{algorithm}[h]
\caption{Compute a textured image for the creation of textured-ADE20K dataset \shai{I think we should remove the Algorithm. It's way too long and does not provide any insights.}
}
\SetAlgoLined
\DontPrintSemicolon
\KwIn{Content image $\contentimage$ from ADE20K, set of texture images $\textureimageset$ from DT, set of instance masks $\maskset$ of $\contentimage$, $|\maskset|=|\textureimageset|$, texture encoder $\encoder$ and decoder $\decoder$}
\KwOut{Textured content image $\modified{\contentimage}$}
$\sizeof{\contentsymbol}\assign\size(\contentimage)$ \;
$\contentimage \assign \scale(\contentimage)\in \realnumberset^{8\imagesize\times8\imagesize}$ \; 
$\textureimage\assign\scale(\textureimage)\in \realnumberset^{\imagesize\times\imagesize}$ \;
Extract overlapping patches $\contentimagepatch\in \realnumberset^{\imagesize\times\imagesize}$,  $\patch \in \patchset$ from $\contentimage$\; 
$\gaussiansetcontent\assign\emptyset$ \;
\For{$\patch \in \patchset$}{
    $\gaussiansetcontentpatch \assign \encoder(\contentimagepatch)$ \;
    $\gaussiansetcontent \assign \gaussiansetcontent \bigcup \gaussiansetcontentpatch$
}
\tcp{see \cite{Tu:2024:CNT} for details about $\merge$}
$\gaussiansetcontent\assign\merge(\gaussiansetcontent)$ \; 
$\modified{\gaussiansetcontent}\assign\emptyset$ \;
\For{$\mask \in \maskset$, $\textureimage \in \textureimageset$}{
    \tcc{modulate Gausisan features within a mask (Maskwise feature modulation)}
    $\gaussiansettexture\assign\encoder(\textureimage)$ \;
    $\contentmasked{\gaussianset}\assign\setof{\gaussiancontent | \gaussiancontent \in \gaussiansetcontent, \mask(\gaussiancenter_\contentsymbol)=1}$ \;
    $\contentmasked{\modified{\gaussianset}} \assign \emptyset$ \;
    \For{$\contentmasked{\gaussian}\in\contentmasked{\gaussianset}$}{
        \tcp{RandomSelect randomly picks an entry from a set}
        $\gaussiantexture\assign$ RandomSelect($\gaussiansettexture$)  \; 
        \tcc{$\contentmasked{\gaussian}\ \textnormal{is} \       \setof{\contentmasked{\appearancefeature},\contentmasked{\gaussiancenter},\contentmasked{\gaussiancovariance}}$  \\       $\gaussiantexture \ \textnormal{is} \       \setof{\appearancefeature_\texturesymbol,\gaussiancenter_\texturesymbol,\gaussiancovariance_\texturesymbol}$
        } 
        $\contentmasked{\modified{\appearancefeature}}\assign\interpcoefficient \contentmasked{\appearancefeature} + (1-\interpcoefficient) \appearancefeature_\texturesymbol$ \;
        $\modified{\contentmasked{\gaussian}}\assign\setof{\contentmasked{\modified{\appearancefeature}},\contentmasked{\gaussiancenter},\contentmasked{\gaussiancovariance}}$ \;
        $\contentmasked{\modified{\gaussianset}}\assign \contentmasked{\modified{\gaussianset}} \bigcup \setof{\contentmasked{\modified{\gaussian}}}$
    }    $\modified{\gaussiansetcontent}\assign\modified{\gaussiansetcontent}\bigcup\contentmasked{\modified{\gaussianset}}$
}
$\modified{\contentimage}\assign\decoder(\modified{\gaussiansetcontent})$ \;
$\modified{\contentimage}\assign \scale(\modified{\contentimage}) \in \realnumberset^{\sizeof{\contentsymbol}}$ \;
\Return $\modified{\contentimage}$
\label{alg:dataset}
\end{algorithm}
